Boosting-based Construction of BDDs for Linear Threshold Functions and Its Application to Verification of Neural Networks

Understanding the characteristics of neural networks is important but difficult due to their complex structures and behaviors. Some previous work proposes to transform neural networks into equivalent Boolean expressions and apply verification techniques for characteristics of interest. This approach is promising since rich results of verification techniques for circuits and other Boolean expressions can be readily applied. The bottleneck is the time complexity of the transformation. More precisely, (i) each neuron of the network, i.e., a linear threshold function, is converted to a Binary Decision Diagram (BDD), and (ii) they are further combined into some final form, such as Boolean circuits. For a linear threshold function with $n$ variables, an existing method takes $O(n2^{\frac{n}{2}})$ time to construct an ordered BDD of size $O(2^{\frac{n}{2}})$ consistent with some variable ordering. However, it is non-trivial to choose a variable ordering producing a small BDD among $n!$ candidates. We propose a method to convert a linear threshold function to a specific form of a BDD based on the boosting approach in the machine learning literature. Our method takes $O(2^n \text{poly}(1/\rho))$ time and outputs BDD of size $O(\frac{n^2}{\rho^4}\ln{\frac{1}{\rho}})$, where $\rho$ is the margin of some consistent linear threshold function. Our method does not need to search for good variable orderings and produces a smaller expression when the margin of the linear threshold function is large. More precisely, our method is based on our new boosting algorithm, which is of independent interest. We also propose a method to combine them into the final Boolean expression representing the neural network.

==> ABDD.tex <==
\section{\our{} Construction}

We now apply the \our{} Boosting algorithm developed in the previous
section to a given linear threshold function $f$ to obtain an
\our{} representation $T$ for $f$.
In particular, we show that the size of $T$ is small when $f$ has a
large margin.

To be more specific, assume that we are given a linear threshold function
$f: \{-1,1\}^n \to \{-1,1\}$ of the form
\[
	f(x) = \sigma(w \cdot x + b)
\]
for some weight vector $w \in \mathbb{R}^n$ and bias $b \in \mathbb{R}$,
where $\sigma$ is the step function, i.e., 
$\sigma(z)$ is $1$ if $z \geq 0$ and $-1$ otherwise.
Note that there are infinitely many $(w,b)$ inducing the same
function $f$. We define the margin $\rho$ of $f$ as the maximum
margin $f(x)(w \cdot x + b)/\|w\|_1$ over all $(w,b)$.
We let our hypothesis set $\calH$ consist of projection functions,
namely, $\calH = \{h_1,h_2,\dots,h_n,h_{n+1}, h_{n+2},\dots,h_{2n}\}$,
where $h_i:x \mapsto x_i$ if $i \leq n$ and $h_i:x \mapsto -x_i$
otherwise, so that we can represent $f$ as
$f(x) = \sigma(\sum_{i=1}^{2n} w_i h_i(x) + b)$ for some
non-negative $2n$-dimensional weight vector $w \geq 0$ and bias $b$.
Then, we can represent the margin $\rho$ of $f$ as the solution of
the optimal solution for the following LP problem:
\begin{align} \label{eq:margin}
& \max_{w,b,\rho} \rho \\
\text{s.t. \quad} &
f(x)(\sum_{i=1}^{2n} w_i h_i(x) + b) \geq \rho
\text{ for any $x \in \{-1,1\}^n$,} \nonumber \\
& w \geq 0, \nonumber \\
& \sum_i w_i = 1. \nonumber
\end{align}

Now we show that $\calH$ actually satisfies $\rho$-WHA for $f$.

\begin{lemma}\label{mainlemma}
Let $f$ be a linear threshold function with margin $\rho$.
then $\calH$ satisfies $\rho$-WHA.
\end{lemma}

\begin{proof}
Let $\rho$ be the optimal solution of (\ref{eq:margin}).
By duality, $\rho$ is identical to the optimal
solution $\gamma$ of the dual problem of (\ref{eq:margin}):
\begin{align*}
	& \min_{d,\gamma} \gamma \\
\text{s.t. \quad} & 
\sum_{x \in \{-1,1\}^n} d_x f(x)h_i(x) \leq \gamma
\text{ for any $i \in [2n]$,} \\
& d \geq 0, \\
& \sum_{x: f(x) = 1} d_x = \sum_{x: f(x) = -1} d_x = 1/2. \\
\end{align*}
Apparently, the optimal $\gamma$ should satisfy
$\gamma = \max_{h \in \calH} \sum_x d_x f(x)h(x)$,
which implies the lemma.
\end{proof}
	

By the lemma and Theorem~\ref{mainth}, we immediately have the following corollary.

\begin{corollary}\label{coroabdd}
Let $f$ be a linear threshold function with margin $\rho$.
Applying the \our{} Boosting algorithm with
the sample
$S = \{(x,f(x)) \mid x \in \{-1,1\}^n\}$
of all ($2^n$) instances,
our hypothesis set $\calH$, and
the precision parameter $\varepsilon = 1/2^n$,
we obtain an \our{} $T$, which is equivalent to $f$
of size $O\left(\frac{n}{\rho^4}(n+\ln(1/\rho))\right)$.
\end{corollary}



==> method.tex <==

\section{Boosting}
\subsection{Problem Setting}
Boosting is an approach to constructing a strongly accurate classifier 
by combining weakly accurate classifiers. 
We assume some unknown target function $f:\{-1,1\}^n \to \{-1,1\}$. 
Given a sample 
$S=((x_1,f(x_1)),\dots,(x_m,f(x_m))) \in (\{-1,1\}^n\times \{-1,1\})^m$
of $m$ instances labeled by $f$ and a precision parameter $\varepsilon$, 
we want to find a classifier $g:\{-1,1\}^n \to \{-1,1\}$ such that 
its training error $\Pr_U\{g(x) \neq f(x)\}\leq \varepsilon$, 
where $U$ is the uniform distribution over $S$. 
We are also given a set $\calH$ of base classifiers from $\{-1,1\}^n$ to $\{-1,1\}$. 
We assume the following assumption which is standard in the boosting literature~\cite{mansour2002}.  
%Boosting  a class of iterative algorithms based on the Weak Hypotheses Assumption (WHA) 
%defined in Definition~\ref{wha} for expressing Boolean function classes
%~\cite{freund1995,kearns1999,schapire1990}.

% 
% Let each input sample dimension represents a different hypothesis $h$, 
% %and each h points to a column of the sample, 
% called an $edge$, denoted as $h(x)$.

\begin{myDef}{(Weak Hypotheses Assumption (WHA))}\label{wha}\\
%A hypothesis set $H_x=\{h:{\{-1,1\}}^n\rightarrow\{-1,1\}|h(x)=x_i \mbox{ for some } i\in \{1,\dots,n\}\}$ 
%satisfies:
%For $\gamma>0$, the $\gamma$-Weak Hypotheses Assumption for the target function $f:{\{-1,1\}}^n\rightarrow\{-1,1\}$.
A hypothesis set $\calH$ satisfies $\gamma$-Weak Hypothesis Assumption (WHA) for the target function 
$f:\{-1,1\}^n \to \{-1,1\}$ 
if 
for any distribution $d$ over $\{-1,1\}^n$, there exists $h\in \calH$ such that 
%If for any distribution $d$ over domain $X={\{-1,1\}}^n$,
%there exists a hypotheses $h\in H_x$, s.t.
$edge_{d,f}(h)\triangleq\sum_{x\in \{-1,1\}^n} d_x f(x) h(x)\geq \gamma$. 
\end{myDef} 
Intuitively, WHA ensures the set of $\calH$ of hypotheses and $f$ are ``weakly'' related to each other. 
The edge function $edge_{d,f}(h)$ takes values in $[-1,1]$ and equals to $1$ if $f=h$. 
Under WHA, we combine hypotheses of $\calH$ into a final hypothesis $h_T$ represented by an ABDD $T$
\footnote{More precisely, here, 
we consider a generalized form of ABDD where each node is labeled by a hypothesis in $\calH$.}.

Our analysis is based on a generalized version of entropy~\cite{kearns1999}. 
A pseudo-entropy $G:[0,1] \to [0,1]$ is defined as $G(q)\defeq2\sqrt{q(1-q)}$. 
Like the Shannon entropy, $G$ is concave and $G(1/2)=1$, and $G(0)=G(1)=0$. 
In particular, $\min(q, 1-q)\leq G(q)$. 
Then we will introduce the conditional entropy of $f$ given a sample $S$ and an ABDD $T$. 
For each node $u$ in $T$, let $p_u \defeq\Pr_U\{\text{$x$ reaches at $u$}\}$ and 
$q_u \defeq\Pr_U\{f(x)=1 \mid \text{$x$ reaches at $u$}\}$, respectively. 
Let $N(T)$ be the set of nodes in $V\setminus L$ whose depth is the maximum. 
We further assume that 
for each node $u$ in $N(T)$, the $x$ in $u$ is assigned to $1$-leaf if $q_u \geq 1/2$, and is assigned to $0$-leaf, otherwise.
Then, observe that $\Pr_U\{f(x)\neq h_T(x)\}=\sum_{u \in N(T)}p_u \min (q_u, 1-q_u)$.  
The conditional entropy of $f$ given an ABDD $T$ w.r.t. the distribution $U$ is defined as 
\begin{equation}\label{eq1}
    \begin{split}
    H_U(f|T)=\sum_{u\in N(T)} p_u G(q_u).
    \end{split}
\end{equation} 
Then the conditional entropy gives an upper bound of the training error as follows.

%When a supervised neural network is trained by instances, the neural network can be seen as a set of linear threshold functions.
%% to predict other untrained data $X^\prime$. 
%Similarly, we use weak learning theory to learn NN from the same instances.
%Given (1) a set of instances
%$S=((x_1,f(x_1)),\ldots,(x_m,f(x_m)))\in (\{-1,1\}^n\times ({-1,1}))^m$, 
%labeled with a function $f:\{-1,1\}^n\rightarrow \{-1,1\}$; 
%(2) $\mathcal{H}\subseteq \{h:\{-1,1\}^n\rightarrow \{-1,1\}\}$ satisfying $\gamma$-WHA 
%with respect to $f$; 
%(3) $\epsilon\in (0,1]$; under uniform distribution $U$, 
%our method output a ABDD $T$ such that training error $err_U(h_T)=Pr_U\{h_T(x)\neq f(x)\}<\epsilon$.


% Our proposed method focuses on finding suitable hypotheses $h$ to split the sample from the parent node by WHA.
    
 

% Note that, in Mansour et al.~\cite{mansour2002}, Definition~\ref{wha} is used for each node of the BDD to learn Boolean functions.

% \begin{flalign}\label{maxmin}
% \begin{matrix}
% &\max_{w,\rho,b} \rho\\
% &s.t.\indent y(w\cdot x+b)\geqslant \rho\\
% &\sum w_j\leqslant 1%\\
% \end{matrix}
% \begin{matrix}
% %\stackrel{\mbox{dual problem}}{\longrightarrow}
% \longrightarrow
% \end{matrix}
% \begin{matrix}
% &\min_d \gamma\\
% s.t. & \indent \sum_{(x,y)\in S} d_{x} f(x) h(x) \leqslant \gamma \\%\mbox{,   } \forall j\in [n]\\
% &\sum_{(x,y)\in S} d_{x}=1\\
% &d_{x}\geqslant 0\\
% \end{matrix}
% \end{flalign}
% where $\gamma$ is the margin of logical function.


%%%%%%%%%%%%%%
% The input of our algorithm are $b\in \mathbb{R}$ and $w\in \mathbb{R}^n$ of linear threshold function $f$, where $\sum{w}=1$. %; error $\epsilon \in (0,1)$ {[0,1]}
% %and $\gamma>0$.
% Using $w$ and $b$, we have sample set $S=\{(x,f(x))|x\in \{-1,1{\}}^n\}$, where $f(x)=sign(w\cdot x+b)$.

%%%%%%%%%%%%%%%%%%%%

% We build BDD and \our based on Mansour et al.~\cite{mansour2002}.
% We assume a decision diagram $T$ with internal nodes and leaf nodes.
% A leaf node has no outgoing edge; an internal node is labeled with hypothesis $h\in H$ 
% and has two outgoing edges, which are marked by $\{-1,1\}$. 
% %Note that nodes in the same layer will be labeled with the same hypothesis $h$ in \our.
% Given sample $S$, each instance $x\in S$ determines the unique path from the root node through 
% each edge of the node and finally reaches a leaf node. 
%Just like the algorithm of the BDD in~\cite{mansour2002},
%we also have split and merge operations at a hidden layer in this paper.
%For a given DD $T$, node $u\in T$ and sample $S$, which contains data $X$ and labels $Y$,
%we write $S_u$ to denote the set of pairs $(x,y)\in S$ such that $x$ reaches $u$.
%We define fraction $p_u=Pr_D(\mbox{instance $x$ reaches at $u$})$ to count how much sample reach the node and $q_u=Pr_D(f(x)=1|\mbox{$x$ reaches at $u$})$ to calculate the proportion of $f(x)=1$ in the sample $S_u$.


%The split depends on hypothesis $h$, proposed in Definition~\ref{wha}, 
%and the merge depends on the interval in Definition~\ref{mydef1}.
%The split nodes with the same $q$ will enter the same interval and merge as a new node.
    


%As for the details of the split part, 
%the key to using the WHA for DD learning is the use of the entropy function. 
%We set the entropy function to be $G(q)=2\sqrt{q(1-q)}$, 
%where $G(q)$ is monotonically increasing on the $[0,1/2]$ and
%monotonically decreasing on $[1/2,1]$.


\begin{prop}\label{propp0}
$\Pr_U\{h_T(x)\neq f(x)\}\leqslant H_U(f|T)$.
\end{prop}
%The proof for Proposition~\ref{propp0} is in the Appendix~\ref{propp0l}.
\begin{proof} 
By using the property that $\min(q,1-q)\leq G(q)$, 
$\Pr_U\{h_T(x) \neq f(x)\}=\sum_{u\in N(T)}p_u \min(q_u,1-q_u) \leqslant \sum_{u\in N(T)}p_uG(q_u)$.
\end{proof} 
Therefore, it is sufficient to find an ABDD $T$ 
whose conditional entropy $H_U(f|T)$ is less than $\varepsilon$.

We will further use the following notations and definitions. 
Given an ABDD $T$, $S$ and $u \in N(T)$, let $S_u=\{(x,y)\in S \mid \text{$x$ reaches at $u$}\}$.
The entropy $H_d(f)$ of $f:\{-1,1\}^n \to \{-1,1\}$ 
w.r.t.~a distribution $d$ over $\{-1,1\}^n$
is defined as $H_d(f)\defeq G(q)$, where $q=\Pr_d\{f(x)=1\}$. 
The conditional entropy $H_d(f|h)$ of $f$ given $h:\{-1,1\}^n \to \{-1,1\}$ w.r.t.~$d$ is defined as 
$H_d(f|h)=\Pr_d\{h(x)=1\}G(q^+) + \Pr_d\{h(x)=-1\}G(q^-)$, 
where $q^{\pm}=\Pr_d\{f(x)=1 \mid h(x)=\pm1\}$, repectively.
\subsection{Our Boosting Algorithm}
Our algorithm is a modification of the boosting algorithm 
proposed by Mansour and McAllester~\cite{mansour2002}.
Both algorithms learn Boolean functions in the form of BDDs in a top-down way.
The difference between these algorithms is that 
ours constructs the final Boolean function with the form of ABDDs, while Mansour and McAllester's is not.
This change might seem to be subtle, but needs a new criterion to choose hypotheses in $\calH$ 
and shows better results in the experiments. 

Our boosting algorithm iteratively grows an ABDD by adding a new layer at the bottom. 
More precisely, at each iteration $k$, given the current ABDD $T_k$, 
the algorithm performs the following two consecutive processes 
(as illustrated in Figure~\ref{hiddenl}).
\begin{description}
    \item[Split:] 
    It chooses a hypothesis $h_k\in \calH$ using some criterion and 
adds two child nodes for each node in $N(T_k)$ in the next layer, 
where each child corresponds to $\pm 1$ values of $h_k$.
Let $T_k'$ be the resulting DD. 
\item[Merge:]
It merges nodes in $N(T_k')$ according to some rule 
and let $T_{k+1}$ be the ABDD after the merge process.
\end{description}

The full description of the algorithm is given in Algorithm~\ref{alg1} and~\ref{algsplit}, 
respectively.
For the split process, it chooses the hypothesis $h_k$ 
maximizing the edge $edge_{\hat{d},f}(h)$ w.r.t.~the distribution $\hat{d}$ specified in 
(\ref{balance_dist}). 
For the merge process, we use the same way in the algorithm of Mansour and McAllester~\cite{mansour2002}.

\begin{myDef}{~\cite{mansour2002}}\label{mydef1} 
For $\delta$ and $\lambda$ ($0<\delta,\lambda <1$),
a $(\delta,\lambda)$-net $\calI$ is defined as 
a set of intervals $[v_0,v_1],[v_1,v_2],\dots,[v_{w-1},v_w]$ such that 
(i) $v_0=0$, $v_w=1$, (ii) for any $I_k=[v_{k-1},v_k]$ and $q \in I_k$, 
$\max_{q' \in I_k}G(q')\leq \max\{\delta, (1+\lambda)G(q) \}$. 
%a set of intervals $I_k$   $\gamma\in \left(0,1/2\right]$.
%The interval point $v\in (0,1)$ is written as \\
%$(0,v_1],[v_1,v_2],\ldots,[v_{i-1},1)\in \mathcal{I}$,
%where $i$ is the number of intervals, and $v_{i/2}=\frac{1}{2}$.
% For each node $u$, there is only one interval $I$ here has $G(q_u)\in I$.
%For $1\leqslant j \leqslant i/2 =\ulcorner\frac{\ln(\frac{1}{\epsilon})}{\ln(1+\gamma)}\urcorner$,
%$v_{\frac{i}{2}-j}$ is defined as $v_{\frac{i}{2}-j}=G^{-1}(\frac{G(\frac{1}{2})}{{(1+\lambda)}^j})$, and 
%the $i/2\leqslant j \leqslant i$ part can be defined similarly.
%Then, we have $G(v_1)\leqslant \epsilon$ and $G(v_{i/2-j})/G(v_{i/2-j-1})=1+\gamma$.
% \begin{equation}\label{eq01}
% \begin{split}
% G(v_1)\leqslant \epsilon,
% \end{split}
% \end{equation}
% \begin{equation}\label{eq02}
% \begin{split}
% G(v_{i/2-j})/G(v_{i/2-j-1})=1+\frac{\hat{\gamma}}{3},
% \end{split}
% \end{equation}
\end{myDef}
Mansour and McAllester showed a simple construction of $(\delta,\lambda)$-net 
with length $w=O((1/\lambda)\ln (1/\delta))$~\cite{mansour2002} and we omit the details.
Our algorithm uses particular $(\delta,\lambda)$-nets for merging nodes.

\subsection{Analyses}


%Similar to the description in~\cite{kearns1999,mansour2002} for calculating the entropy difference in each node,
%this is easy to define the entropy difference computation 
%within each depth in \our. 
%We define the set of nodes at depth $k$ as $\mathbf{L}_k$. 
%When the sample reaches the node $u\in \mathbf{L}_k$ with sample $S_u$, at the depth $k$.
%Let $\ell_k:X \rightarrow \mathbf{L}_k$ denote the function that maps an instance $x$ to the node in $\mathbf{L}_k$ on the path that $x$ induces. 
%We set a function $H_d(Y|\ell_k)$ to be the total conditional G-entropy of $Y$ at depth $k$ of \our{} under any distribution $d$.\@
%\begin{equation}\label{eq1}
%\begin{split}
%H_d(Y|\ell_k)=\sum_{u\in \mathbf{L}_k} p_u G(q_u),
%\end{split}
%\end{equation}
%where $p_u=Pr_d(\mbox{instance $x$ reaches at $u$})$ and $q_u=Pr_d(f(x)=1|\mbox{$x$ reaches at $u$})$

%Similarly, we also define $H_d(Y|\ell_k,h)$ to be the entropy after split as follows:
\begin{equation}\label{eq2}
\begin{split}
H_d(Y|T,h)=\sum_{u\in N(T)} (p_{u^+} G(q_{u^+})+p_{u^-} G(q_{u^-}))
\end{split}
\end{equation}
where $p_{u^\pm}=Pr_d\{x \mbox{ reaches at }u | h(x)=\pm1\}$ and 
$q_{u^+}=Pr_d(f(x)=1|\mbox{$x$ reaches at $u$, $h(x)=1$})$. $p_{u^-}$ and $q_{u^-}$ are defined similarly.

% where $p_{u^+}=p_u \frac{|{(x,y)\in S_u|h(x)=1}|}{|S_u|}=p_u \frac{|S_{u^+}|}{|S_u|}$ 
% and $q_{u^+}=\frac{|{(x,y)\in S_u|h(x)=1}|}{|S_{u^+}|}$. $p_{u^-}$ and $q_{u^-}$ is defined similarly.

% When the sample under the distribution $D$, 
% the sum of the entropy at $\mathbf{L}_k$ is $H_D(Y|\ell_k)$, 
% then $H_D(Y|h,\ell_k)$ is the sum of the entropy at $\mathbf{L}_k$ split by 
% hypotheses $h$. 

% Therefore, We define the entropy difference $\triangle(S_u,h)$ due to the split as follows:
% \begin{equation}\label{eq3}
% \begin{split}
% \triangle(S_u,h)&=H(Y|\ell_k)-H(Y|\ell_k,h)\\
% &=\sum_{u\in \mathbf{L}_k} p_u (G(q_u)-\frac{|S_{u^+}|}{|S_u|} G(q_{u^+})-\frac{|S_u^-|}{|S_u|} G(q_{u^-}))
% \end{split}
% \end{equation}


% \begin{equation}\label{eq001}
% \begin{split}
% v_{\frac{i}{2}-j}=G^{-1}(\frac{G(\frac{1}{2})}{{(1+\frac{\hat{\gamma}}{3})}^j}).
% \end{split}
% \end{equation}



% Due to the property of the entropy function, it's easy to see that the interval will 
% gradually become wider within $[0,1/2]$ and narrower within $[1/2,1]$.
% $v_1$ is the largest $v$ less than $\epsilon$ and $\mathcal{I}_k$ means the set of 
% all intervals at $k$-th layer.


% Due to Mansour et al.~\cite{mansour2002}, the following results give us an upper bound on 
% the size of the BDD generated by the weak learning hypothesis.

% \begin{theorem}{(Mansour et al.~\cite{mansour2002})}\label{def01} 
% Assuming the $\gamma$-weak index reduction hypothesis, 
% a linear threshold classifier in the 
% form of eq~\ref{bnnunit} can be represented by a BDD of 
% size $O(\frac{1}{\rho^2}\ln{\frac{1}{\rho^2}})$ nodes,
% where $\rho$ is the margin of the linear threshold classifier.
% \end{theorem}

% Observing Definition~\ref{def01}, 
% we can see that the larger the margin of the linear threshold classifier, 
% the smaller the BDD we obtain.
% In fact, this definition is also applicable to our \our.

% Define the balanced distribution of sample $(x,y)\in S$ as follows:
% \begin{equation}\label{balancedd}
% \begin{split}
% d_{(x,y)}=
% \begin{cases} 
% \frac{1}{2\times |\{(x^\prime,y^\prime)\in S|y=1\}|}, & \mbox{if }y=1 \\
% \frac{1}{2\times |\{(x^\prime,y^\prime)\in S|y=-1\}|}, & \mbox{if }y=-1
% \end{cases}
% \end{split}
% \end{equation}

The following lemmas prove an effective weak learning algorithm 
under a variant balanced distribution $\bar{d}$, and it also can be achieved 
under any distribution. For $(x,y)\in S$:
\begin{equation}\label{vbalancedd}
\begin{split}
\bar{d}_{(x,y)}=
\frac{d_{(x,y)}}{2\sum_{(x^\prime,y) \in S} d_{(x^\prime,y)}}
\end{split}
\end{equation}


\begin{lemma}{\cite{takimoto2003}}\label{lemma1-1}
%Let $f:X\rightarrow\{-1,1\}$. 
Let $d$ and $\bar{d}$ be any distribution over $\{-1,1\}^n$ 
and its balanced distribution w.r.t. some $f:\{-1,1\}^n \to \{-1,1\}$, 
respectively.
Then, for any hypothesis with $edge_{\bar{d},f}(h)\geq \gamma$, 
%conditional entropy of $Y$ given $h$ with respect to $d$ have
$H_{d}(f|h)\leqslant(1-\gamma^2/2)H_{d}(f)$.
\end{lemma}

%\begin{lemma}{\cite{takimoto2003}}\label{lemma1}
% Assume that $G$ is used for the pseudo-entropy function.
% If there exists a weak learning algorithm with respect to balanced distributions, 
% then there exists a distribution-free weak learning algorithm.
%Under any distribution $d$, the entropy function $G$ of $Y$ has $H_d(Y)\leqslant H_{\bar{d}}(Y)$.
%\end{lemma}


Based on Lemma~\ref{lemma1-1}, we establish the connection between $\gamma$ 
and entropy function, and have a $\gamma^*\in (0,1)$ at each depth to reflect the entropy change
under our algorithm.

\begin{lemma}\label{lemma0} 
Let $\hat{d}$ be the distribution over $S$ specified in (\ref{balance_dist}) 
when $T_k$, $\calH$ and $S$ is given by Algorithm~\ref{algsplit} and let $h_k$ be the output.
If $\calH$ satisfies $\gamma$-WHA, 
then %there exists some $h\in \calH$ such that  %$edge_{d,f}(h)\geq \gamma$, for a distribution $d$, 
the conditional entropy of $f$ w.r.t. the distribution $U$ over $S$ given $T_k$ and $h_k$ is bounded as 
$H_U(f|h_k,T_k)\leqslant (1-\gamma^{2}/2)H_U(f|T_k)$.
\end{lemma}

% The proof for Lemma~\ref{lemma0} is in the Appendix~\ref{lemma0l}.

\begin{proof}
%eq 456
For $(x,y) \in S_u$, we define the balanced distribution of node $u$ as follows:
\begin{equation}\label{eq12}
\begin{split}
d_{(x,y)}^u=
\begin{cases} 
\frac{1}{2\times |\{(x^\prime,y^\prime)\in S_u|y=1\}|},  & \mbox{if }y=1  ~\&  ~(x,y)\in S_u\\
\frac{1}{2\times |\{(x^\prime,y^\prime)\in S_u|y=-1\}|}, & \mbox{if }y=-1 ~\&  ~(x,y)\in S_u\\
0, & \mbox{if } (x,y)\notin S_u
\end{cases}
\end{split}
\end{equation}
%Note that, when there is no $y=1$ or $y=-1$ in $S$, we set the corresponding value to 0.



Under the balanced distribution $d^{u}$, let 
\begin{equation}\label{eq11}
\begin{split}
\gamma_{u,h_k}=edge_{d^u,f}(h_k)
%\sum_{(x,y)\in S_u} d_{(x,y)}^u y h(x)
\end{split}
\end{equation}
be the edge of $h_k$ w.r.t. $d^u$ and $f$. 
%\lVert w\rVert
By Lemma~\ref{lemma1-1}, we have
\begin{equation}\label{eq4}
\begin{split}
H_{d^u}(f|h)\leqslant (1-\gamma^2_{u,h}/2)H_{d^u}(f).
\end{split}
\end{equation}

%Let $H(Y|h,\ell(x)=u)$ be the conditional G-entropy of $Y$ after instance $x$ reach node $u$ and split by hypotheses $h$.

\begin{equation}\label{eq5}
\begin{split}
H_{d^u}(Y|h)=H_{d}(Y|h,\ell_k(x)=u)\leqslant (1-\frac{\gamma^2_{u,h}}{2})H_{d^u}(Y)
\end{split}
\end{equation}


% By definition of $\ell_k$ and distribution $D_u$, 
% we can have
% \begin{equation}\label{eq5-1}
% \begin{split}
% H_{D^u}(Y|h,\ell_k)=H(Y|h,\ell_k(x)=u)
% \end{split}
% \end{equation}

%We apply Lemma~\ref{lemma1}, extending the problem from 
%the balanced distribution to any distribution.

% When we observe the total entropy change of the $k$-th layer,
% we have 
%\begin{small}
Thus, 
\begin{equation}\label{eq5-2}
\begin{split}
H_U(f|h_k,T_k)
=&\sum_{u \in N(T_k')}p_u G(q_u)\\
=&\sum_{u \in N(T_k)}H_{d^u}(f|h_k)\\
%\sum_{u\in\mathbf{L}_k}p_u H_{d^u}(Y|h,\ell_k (x)=u)=H_D(Y|h,\ell_k)\\
\leq& \sum_{u\in N(T_k)}p_u(1-\gamma^2_{u,h_k}/2)H_{d^u}(f)\\
=&\sum_{u\in N(T_k)}p_u H_{d^u}(f)\\
 & -\sum_{u\in N(T_k)}p_u \frac{\gamma_{u,h}^2}{2}H_{d^u}(f)\\
=&H_U(f|T_k)-\sum_{u\in N(T_k)}p^\prime_u \frac{\gamma_{u,h_k}^2}{2}H_{U}(f|T_k),
\end{split}
\end{equation}
%\end{small}
%By definition, we can rewrite eq~\ref{eq1}, and have
where 
$p^\prime_u =p_u \frac{H_{d_u}(f)}{H_U(f|T_k)}
=p_u\frac{G(q_u)}{\sum_{u\in N(T_k)}p_u G(q_u)}$ 
which is specified in line $3$ of Algorithm~\ref{algsplit}.
% \begin{equation}\label{eq13}
% \begin{split}
% p^\prime_u =p_u \times \frac{H_{D_u}(Y)}{H(Y|\ell_k)}=p_u\times\frac{G(q_u)}{\sum_{u\in \mathbf{L}_k}p_u G(q_u)}.
% \end{split}
% \end{equation}


Here, we define a distribution $\hat{d}$ for samples in node $u$.
\begin{equation}\label{eq13-1}
\begin{split}
\hat{d}_{(x,y)}=\sum_{u\in N(T_k)} p^\prime_u d_{(x,y)}^u
\end{split}
\end{equation}


By using (\ref{eq5-2}), (\ref{eq13-1}), $\gamma$-WHA, and Jensen's inequality, 
we get
\begin{equation}\label{eq14}
\begin{split}
\sum_{u\in N(T_k)} p^\prime_u\gamma_{u,h_k}^2 
&=\sum_{u\in N(T_k)} p_u^\prime {(\sum_{(x,y)\in S_u} d_{(x,y)}^u y h_k(x))}^2\\
&\geqslant{(\sum_{u\in N(T_k)} p_u^\prime \sum_{(x,y)\in S_u} d_{(x,y)}^u y h_k(x))}^2\\
&={(\sum_{u\in N(T_k)} \sum_{(x,y)\in S_u} p_u^\prime d_{(x,y)}^u y h_k(x))}^2\\
%&={(\sum_{u\in \mathbf{L}_k} \sum_{(x,y)\in S_u} \hat{d}_{(x,y)}^u y h(x))}^2\\
&={(\sum_{(x,y)\in S} \hat{d}_{(x,y)} y h_k(x))}^2\\
&=(edge_{\hat{d},f}(h_k))^2\\
&\geqslant{\gamma}^2.
\end{split}
\end{equation}

By combining \eqref{eq5-2} and \eqref{eq13-1}, 
\eqref{eq14} can be rewritten as 
\begin{equation}\label{eq5-3}
\begin{split}
H_U(f|h_k,\ell_k)
%&\leqslant H_U(f|T_k)-\sum_{u\in N(T_k)}p^\prime_u \frac{\gamma^2_{u,h}}{2}H_D(Y|\ell_k)\\
&\leqslant (1-\gamma^{2})H_U(f|T_k)
\end{split}
\end{equation}
as desired.
\end{proof}

    

%From Lemma~\ref{lemma0}, we have $H_D(Y|h,\ell_k)\leqslant (1-\frac{\gamma_{*,h}^2}{2})H_D(Y|\ell_k)$ and $\gamma=\frac{\hat{\gamma}}{3}$, where
%$\hat{\gamma}$ is denoted as follows:
%\begin{small}
%\begin{equation}\label{eq5-4}
%\begin{split}
%\hat{\gamma}&\leqslant 2\times(1-\frac{H_D(Y|h,\ell_k)}{H_D(Y|\ell_k)})\\
%&=2\times(1-\frac{\sum_{u\in\mathbf{L}_k}p_{u^+}G(q_{u^+})+p_{u^-}G(q_{u^-})}{\sum_{u\in\mathbf{L}_k} p_u G(q_u)})
%\end{split}
%\end{equation}
%\end{small}


\begin{lemma}{(\cite{mansour2002})}\label{lemma-merge} 
    Assume that, before the merge process in Algorithm~\ref{alg1}, 
    $H_U(f|h_k,T_k)\leq (1-\lambda) H_U(f|T_k)$ for some $\lambda$ ($0<\lambda<1$). 
    Then, by merging based on the $(\delta, \eta)$-net with 
    $\delta=(\lambda/6)H_U(f|T_k)$ and $\eta=\lambda/3$, 
    %Let $\hat{d}$ be the distribution over $S$ specified in (\ref{balance_dist}) 
    %when $T_k$, $\calH$ and $S$ is given to Algorithm~\ref{algsplit} and let $h_k$ be the output.
    %If $\calH$ satisfies $\gamma$-WHA, 
    %then %there exists some $h\in \calH$ such that  %$edge_{d,f}(h)\geq \gamma$, for a distribution $d$, 
    the conditional entropy of $f$ w.r.t. the distribution $U$ over $S$ given $T_{k+1}$ is bounded as 
    $H_U(f|T_{k+1})\leqslant (1-\lambda/2)H_U(f|T_k)$, 
    where the width of $T_{k+1}$ is $O((1/\lambda)(\ln(1/\lambda)+\ln(1/\varepsilon)))$, 
    provided that $H_U(f|T_k)>\varepsilon$.
    \end{lemma}
    

%From this, we sort out the following sub-algorithm~\ref{algsplit} and algorithm~\ref{alg1} to generate a \our{} as shown in Figure~\ref{hiddenl}.\@
% The input of our algorithm are $b\in \mathbb{R}$ and $w\in \mathbb{R}^n$ of linear threshold function $f$, where $\sum{w}=1$. %; error $\epsilon \in (0,1)$ {[0,1]}
% %and $\gamma>0$.

\begin{algorithm}[h]
\caption{\our{} Boosting}\label{alg1} 
\hspace*{0.02in} {\bf Input:}
a sample $S\in (\{-1,1\}^n\times ({-1,1}))^m$ of $m$ instances by $f$, 
and a set $\calH$ of of hypotheses, and precision parameter $\varepsilon$ ($0<\varepsilon<1$);\\
%\hspace*{0.7in}s.t. $\exists w\in \triangle_n,\exists b\in R, \exists \rho>0$;\\
\hspace*{0.02in} {\bf Output:}
\our{} $T$;%, $\mathbf{h}\in$ \our{} consistent with $S$;
\begin{algorithmic}[1] 
\STATE initialization: $T_1$ is the ABDD with a root and $0,1$-leaves, $k=1$. 
\REPEAT
%%\STATE $\tilde{\mathbf{L}_k},j^*_k=Split(\mathbf{L}_k,n)$
\STATE (\textbf{Split}) Let $h_k=Split(T,\calH,S)$ and add child nodes with each node in $N(T_k)$. 
Let $T_k'$ be the resulting ABDD.

%%%%%%%%%%%%%%%
% \IF{$q_{u^+}$}
% \STATE Let $u_+$ to 1-leaf
% %\ELSIF{$q_{u^-}$}
% %\STATE Let $u^-$ to 0-leaf
% \ELSE
% \STATE erew
% \ENDIF
%\STATE set $z=\{0,1\}$ 
\FOR{$u\in N(T_k')$}
\STATE merge $u$ to the $0$-leaf (the $1$ leaf) if $q_u=0$ ($q_u=1$, resp.).
\ENDFOR

\STATE (\textbf{Merge}) Construct a $(\hat{\delta},\hat{\lambda/3})$-net $\calI_k$ with %calculate interval set $\mathcal{I}_k$ by $\hat{\gamma}$
\STATE 
$\hat{\lambda}=1-\frac{H_U(f|T_k,h_k)}{H_U(f|T_k)}$, 
and $\hat{\delta}=\frac{\hat{\lambda} H_U(f|T_k)}{6}$.
\FOR{$I\in \mathcal{I}_k$} 
\STATE merge all nodes $u \in N(T_k')$ such that $q_u \in I$.
%\STATE $\mathcal{U}_I^+=\{u\in \mathbf{L}_k|q_{u^+}\in I\}$
%\STATE $\mathcal{U}_I^-=\{u\in \mathbf{L}_k|q_{u^-}\in I\}$
%\IF{$\mathcal{U}_I^+\cup \mathcal{U}_I^-\neq \varnothing$}
%\STATE make a new node $v$ with new $\begin{cases}1-edge:\{(u,v)|u\in \mathcal{U}_I^+\}\\(-1)-edge:\{(u,v)|u\in \mathcal{U}_I^-\}\end{cases}$
%\STATE $S_v=\bigcup_{u\in \mathcal{U}_I^-\cup \mathcal{U}_I^+}S_u$
\ENDFOR
\STATE Let $T_{k+1}$ be the resulting ABDD and update $k \leftarrow k+1$. 
\UNTIL{$H_U(f|T_k)<\varepsilon$}
\STATE Output $T=T_k$.
\end{algorithmic} 
\end{algorithm}
%Notation that, 
%$T_k$ is defined as the part of a \our{} $T$ from the root node to depth $k$.
%$u^+$ is a set composed of samples with $x_h=1$ in node $u$, 
%$u^-$ is a set composed of samples with $x_h=-1$ in node $u$, where $x\in S_u$.
% $q_{u^+}$ is calculated as $q_{u^+}=\frac{|(x,y)\in S_{u^+,k}|y=1|}{|S_{u^+,k}|}$,
% and $p_{u^+}$ is calculated as $p_{u^+}=p_u \frac{|{(x,y)\in S_{u}|h(x)=1}|}{|S_{u}|}=p_u \frac{|S_{u^+}|}{|S_u|}=\frac{|S_{u^+}|}{|S|}$.
% $p_{u^-}$ and $q_{u^-}$ are defined similarly.


\begin{figure*}[h]
\begin{center}
\includegraphics[scale=0.2]{splitandmerge.png} 
\caption{Illustration of our boosting algorithm. 
The blue dotted line part represents the process of merging the split temporary nodes into new nodes by searching the equivalence space
that does not appear in the \our. 
Following algorithm~\ref{alg1}, we find some hypothesis $h$ to construct child nodes in the new layer
and then merge nodes afterward.}\label{hiddenl}
\end{center}
\end{figure*}


\begin{algorithm}[h]
\caption{Split}\label{algsplit} 
\hspace*{0.02in} {\bf Input:}
ABDD $T$, a set $\calH$ of hypotheses, a set $S$ of $m$ instances labeled by $f$;\\
\hspace*{0.02in} {\bf Output:}
%%$\tilde{\mathbf{L}_k},j^*_k$
$h \in \calH$;
\begin{algorithmic}[1] 
\FOR{$u\in N(T)$}
\STATE Let \\
$d_{(x,y)}^u=
\begin{small}
\begin{cases} 
\frac{1}{2\times |\{(x^\prime,y^\prime)\in S_u|y=1\}|},  & \mbox{if }y=1  ~\&  ~(x,y)\in S_u\\
\frac{1}{2\times |\{(x^\prime,y^\prime)\in S_u|y=-1\}|}, & \mbox{if }y=-1  ~\&  ~(x,y)\in S_u\\
0, & \mbox{if } (x,y)\notin S_u
\end{cases}
\end{small}$, for $(x,y)\in S$.
\STATE $p^\prime_u =\frac{p_u G(q_u)}{\sum_{u\in \mathbf{L}_k}p_u G(q_u)}$
\STATE Let 
\begin{align}
    \hat{d}_{(x,y)}=\sum_{u\in N(T)}p^\prime_u d^u_{(x,y)} 
    \label{balance_dist}
\end{align}
for $(x,y)\in S$.
\ENDFOR
%\FOR{$i=1$ to $n$}
%%\STATE  $\rho_{i,k}^2=(\sum_{u\in \mathbf{L}_k} \sum_{(x,y)\in S_{u,k}} \hat{d}_{(x,y)}^u y h_i(x))^2$  \hfill($\hat{d}$ from eq~\ref{eq14});
%\STATE $\rho_{i}=\left\vert \sum_{(x,y)\in S} \hat{d}_{(x,y)} y x_i \right\vert$
%\ENDFOR
\STATE Output $h=\arg\max_{h' \in \calH}edge_{\hat{d},f}(h)$.
%()\sum_{(x,y)\in S} \hat{d}_{(x,y)} y h(x) $.
\end{algorithmic} 
\end{algorithm}
    
%By definition, since the part of interval generation and merging of 
%\our{} is similar to~\cite{mansour2002}, 
%we have the following theorem.

Now we are ready to show our main theorem.

\begin{theorem}\label{mainth}
Given a sample $S$ of $m$ instances labeled by $f$, 
and a set $\calH$ of hypotheses satisfying $\gamma$-WHA, 
Algorithm~\ref{alg1} outputs an ABDD $T$ such that 
$\Pr_U\{h_T(x)\neq f(x)\}\leq \varepsilon$. 
The size of $T$ is $O((\ln (1/\varepsilon)/\gamma^4)( \ln (1/\varepsilon) + \ln(1/\gamma)))$ and 
the running time of the algorithm is $\text{poly}(1/\gamma, n)m$.
%The algorithm under $\gamma$-WHA can be run in a way that satisfies
%the size of \our{} is $O(\frac{1}{\gamma^2}\ln (\frac{1}{\gamma^2}))$.
\end{theorem}   
%The proof for Theorem~\ref{mainth} is in Appendix~\ref{thl}.
\begin{proof}
By definition of $\hat{\lambda}$ in Algorithm~\ref{alg1}, 
we have $H_U(f|T_k,h_k)=(1-\hat{\lambda})H_U(f|T_k)$ at each iteration $k$.
Therefore, by Lemma~\ref{lemma-merge}, 
$H_U(f|T_{k+1})\leq (1-\hat{\lambda}/{2})H_U(f|T_k)$. Furthermore, $\hat{\lambda}$ is always larger than 
$\gamma^2/2$, implying that 
$H_U(f|T_{k+1})\leq (1-\gamma^2/{4})H_U(f|T_k)$.
Then, after $K$ iterations, we have 
\begin{align*}
 H_U(f|T_K) 
 \leq \left(1-\frac{\gamma^2}{4}\right)^K \leq e^{-\frac{K\gamma^2}{4}},   
\end{align*}
as $H_U(f)\leq 1$. 
Thus, $K=O((1/\gamma^2)\ln(1/\varepsilon))$ iterations suffices to ensure that 
$\Pr_U\{h_T(x)\neq f(x)\}\leq \varepsilon$.
Since the width of the ABDD $T$ is 
$O((1/\gamma^2)(\ln(1/\gamma)+\ln(1/\varepsilon)))$ by Lemma~\ref{lemma-merge} and 
its depth is $K$, the size is bounded by 
$O((\ln (1/\varepsilon) /\gamma^4) (\ln(1/\varepsilon) +\ln (1/\gamma) ))$, as claimed.
%By Definition~\ref{mydef1}, 
%For each depth in \our, we have width $\bar{w}=2+2\ulcorner\frac{\ln(\frac{1}{\epsilon})}{\ln(1+\gamma)}\urcorner$.
%Using the inequality $\beta \ln(1+\alpha)\geqslant \alpha \ln(1+\beta)$,
%for $\gamma\leqslant 1/2$, we have
%\begin{equation}\label{theq1}
%\begin{split}
%\bar{w}&=2+2\ulcorner\frac{\ln(\frac{1}{\epsilon})}{\ln(1+\gamma)}\urcorner\\
%&\leqslant 4+2\frac{\ln(\frac{1}{\epsilon})}{\ln(1+\gamma)}\\
%&\leqslant 4+\frac{\ln(\frac{1}{\epsilon})}{\ln(3/2)}\\
%&\leqslant 4+\frac{3\ln(\frac{1}{\epsilon})}{\gamma}
%\end{split}
%\end{equation}

%Following the set of $\epsilon$ in Algorithm~\ref{alg1}, 
%for the depth $j$ in \our, we have 
%\begin{equation}\label{theq2}
%\begin{split}
%\bar{w}_{j+1}\leqslant\frac{3}{\gamma}\ln(\frac{1}{G(T_j)})+c,
%\end{split}
%\end{equation}
%where $c$ is independent of $j$ and is $O(\frac{1}{\gamma}\ln(\frac{1}{\gamma}))$.

%By Lemma~\ref{lemma0}, the entropy difference between adjacent depthes is related by $G(T_{j+1})\leqslant (1-\frac{3}{2}\gamma)G(T_j)$.
%It's easy to say $G(T_j)\leqslant{(1-3\gamma)}^j$.

%Under the fact that size of \our{} $|T_{j+1}|=|T_j|+\bar{w}_{j+1}$,
%we can have $|T|$ is bounded by $O(\frac{1}{\gamma}{\ln(\frac{1}{\gamma})}^2)$.
\end{proof}

% \subsection{About BDD construction}

% For the split part in the BDD algorithm, 
% we simplify eq~\ref{eq3} to find the hypothesis $h_u$ that can cause 
% the maximum entropy reduction at node $u$.

% For each $u\in \mathbf{L}_k$, we have
% \begin{equation}\label{eq102}
% \begin{split}
% h_u=\max_h \triangle(S_u,h).
% \end{split}
% \end{equation}
% From eq~\ref{eq10}, we relate the linear threshold function to the BDD algorithm.
% By repeatedly using eq~\ref{eq102}, 
% we obtain the hypothesis that entropy reduction is the largest 
% for each node up to the leaf nodes.


% Then, in order to obtain a certain $\gamma$, by definition and for each
% $u\in \mathbf{L}_k$, we have
% \begin{equation}\label{eq100}
% \begin{split}
% p_{u}^+ G(q_{u}^+)+p_{u}^- G(q_{u}^-)\triangleq (1-\gamma)G(q_u).
% \end{split}
% \end{equation}

% Therefore, we take the smallest $\gamma$ in the layer node as 
% the $\hat{\gamma}$ used to generate the interval for that layer.

% \begin{equation}\label{eq101}
% \begin{split}
% \hat{\gamma}=\min_u \gamma_u=\frac{G(q_u)-(p_{u}^+ G(q_{u}^+)+p_{u}^- G(q_{u}^-))}{G(q_u)}
% \end{split}
% \end{equation}

% Then we use the interval part of algorithm~\ref{alg1} to merge nodes.




